Hyperbolic tessellations associated to Bianchi groups

Let F/Q be number field. The space of positive definite binary Hermitian forms over F form an open cone in a real vector space. There is a natural decomposition of this cone into subcones, which descend give rise to hyperbolic tessellations of 3-dimensional hyperbolic space by ideal polytopes. We compute the structure of these polytopes for a range of imaginary quadratic fields.

==> macros.tex <==
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage[line,color,poly,all]{xy}
\usepackage{graphicx,url,xy,amssymb,booktabs}
\usepackage[noadjust]{cite}
\usepackage{xspace}

%Rings and Fields
\newcommand{\RR}{\mathbb R}%Reals
\newcommand{\ZZ}{\mathbb Z}%Integers
\newcommand{\QQ}{\mathbb Q}%Rationals
\newcommand{\CC}{\mathbb C}%Complex
\newcommand{\FF}{\mathbb F}%Complex
\newcommand{\z}{\zeta}%
\newcommand{\uu}{\mathbf u}%
\newcommand{\OO}{\mathcal O}%Ring of integers
\newcommand{\cC}{\mathcal{C}}
\newcommand{\bcC}{\bar{\cC}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fc}{\mathfrak{c}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\sd}{{\sqrt{d}}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\PP}{\mathbb{P}}

%groups
\newcommand{\group}[1]{\mathbf{#1}}%Algebraic groups
\DeclareMathOperator{\SL}{SL}%Special linear
\DeclareMathOperator{\SO}{SO}%Special Orthogonal
\DeclareMathOperator{\GL}{GL}%General linear
\DeclareMathOperator{\Mat}{Mat}%Special linear  
\DeclareMathOperator{\Gal}{Gal}%Galois  
\DeclareMathOperator{\Sym}{Sym}%Symmetic  

\newcommand{\bG}{\group{G}}
\newcommand{\Gb}{\bar{\Gamma}}
\DeclareMathOperator{\Herm}{Herm}

%Misc. operators etc.
\DeclareMathOperator{\Eis}{Eis}%Eisenstein
\newcommand{\V}{\mathcal{V}}
\newcommand{\q}[2]{\left(\frac{#1}{#2}\right)}%
\newcommand{\del}{\partial}%boundary
\DeclareMathOperator{\rank}{rank}%Rank
\DeclareMathOperator{\Jac}{Jac}%Jaobian
\DeclareMathOperator{\Tr}{Tr}%trace
\DeclareMathOperator{\Res}{Res}%Restriction of scalars
\DeclareMathOperator{\Norm}{N}%Norm
\newcommand{\norm}{\Norm_{F/\QQ}}
\newcommand{\fh}{\mathfrak{h}}
\renewcommand{\Re}{\operatorname{Re}}%Real
\renewcommand{\Im}{\operatorname{Im}}%Imaginary
\newcommand{\ip}[1]{\left \langle #1 \right \rangle}%Inner product
\DeclareMathOperator{\vcd}{vcd}%Virtual cohomolgical dimension
\newcommand{\isomto}{\overset{\sim}{\rightarrow}}%"Isomorphic to" arrow
\DeclareMathOperator{\pr}{pr}%Projection
\DeclareMathOperator{\sgn}{sgn}%Sign
\DeclareMathOperator{\diag}{diag}%diag
\DeclareMathOperator{\Cone}{Cone}%Cone
\newcommand{\Vor}{Vorono\"{\i}\xspace}% Voronoi
\newcommand{\pphi}{\hat{\phi}} %Tr \circ \phi 
\DeclareMathOperator{\frob}{Frob}%Sign
\DeclareMathOperator{\disc}{disc}%discriminant
\newcommand{\tE}{\tilde{E}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\hp}{\mathfrak{H}}
\renewcommand{\d}{\frac{d}{dx}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\lsp}[1]{{}^{#1}\!}%Superscript on the left
%Stabilizer groups
\DeclareMathOperator{\Stab}{Stab}%Stabilizer

%Sets of rational parabolic subgroups/associated vectors
\newcommand{\I} {{\mathcal I}}%Picard Modular (\SU(2,1))
\newcommand{\J} {{\mathcal J}}%Picard Modular

%Vectors and matrices
\newcommand{\vect}[1]{\begin{bmatrix} #1 \end{bmatrix}}%In order to make vectors
\newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix}}%

%Itemize in theorems
\renewcommand{\theenumi}{\roman{enumi}}%Saper's suggestion
\renewcommand{\labelenumi}{(\theenumi)}%Saper's suggestion


%Theorem style and numbering convention
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem*{remark}{Remark}
\newtheorem*{question}{Question}

